Profit Shifting and International Tax Reforms

International taxation rules are outdated, allowing multinationals to shift profits to tax havens. This paper examines how tax reforms affect profit shifting and cross-country welfare. We propose a model that separates real economic profits from paper profits, introducing 'triangle identities' to estimate bilateral profit-shifting flows. Using macro- and firm-level data, paper profits' elasticity is three times that of the tax base. Global minimum tax reforms improve welfare by increasing public goods funding and reducing tax competition. We also identify optimal minimum rates under various taxing-right scenarios and demonstrate that unilateral destination-based-cash-flow-tax reforms' welfare effects depend highly on trade imbalances.

==> Graph/mintax_hq_multi_decompo_rev_all_15.tex <==
\begin{table}[tbp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Multilateral HQ minimum taxation at 15\%: change in tax revenues}
\label{mintax_hq_multi_decompo_rev_all_15}
\begin{tabularx}{\linewidth}{lCCCC}

\toprule
{Country}&{$ \Delta $ Tax revenues (in \%) }&{Tax rate contribution}&{Profit shifting contribution}&{Production relocation contribution} \tabularnewline
\midrule \addlinespace[\belowrulesep]
AUS&1.33&.3&1&.04 \tabularnewline
AUT&3.42&1.15&2.22&.05 \tabularnewline
BEL&5.49&3.95&1.04&.5 \tabularnewline
BGR&3&0&3.24&-.24 \tabularnewline
CAN&3.53&.81&2.73&-.02 \tabularnewline
CHE&-1.39&0&-2.2&.03 \tabularnewline
CHN&.83&.16&.84&-.17 \tabularnewline
CZE&2.89&.88&1.91&.11 \tabularnewline
DEU&3.38&1.57&1.66&.14 \tabularnewline
DNK&4.17&2.14&1.8&.24 \tabularnewline
ESP&3.31&.81&2.51&-.02 \tabularnewline
FIN&5.97&2.81&3.05&.11 \tabularnewline
FRA&5.85&2.49&3.26&.1 \tabularnewline
GBR&5.39&3.07&2.11&.2 \tabularnewline
GRC&3.3&.52&3.24&-.46 \tabularnewline
HKG&-4.64&0&-8.95&-.04 \tabularnewline
HRV&4.53&.97&3.56&0 \tabularnewline
HUN&6.25&3.56&2.4&.29 \tabularnewline
IND&1.45&.07&1.63&-.25 \tabularnewline
IRL&-2.88&0&-10.63&.09 \tabularnewline
ISR&1.74&.25&1.68&-.19 \tabularnewline
ITA&3.39&.77&2.69&-.07 \tabularnewline
JPN&2&.35&1.82&-.16 \tabularnewline
KOR&.94&.26&.72&-.04 \tabularnewline
LTU&1.33&0&1.41&-.08 \tabularnewline
LUX&-3.21&0&-19.53&.09 \tabularnewline
MEX&1.14&.06&1.2&-.11 \tabularnewline
MYS&1.21&.35&.82&.04 \tabularnewline
NLD&-6.33&0&-17.15&0 \tabularnewline
NOR&1.65&.55&.95&.15 \tabularnewline
NZL&1.63&.17&1.66&-.19 \tabularnewline
OFC&-4.9&0&-33.74&.08 \tabularnewline
POL&1.88&.18&1.78&-.08 \tabularnewline
PRT&2.21&.19&2.16&-.15 \tabularnewline
RUS&1.22&.18&1.2&-.16 \tabularnewline
SGP&-2.71&0&-6.26&.02 \tabularnewline
SVK&1.95&.27&1.66&.03 \tabularnewline
SWE&7.23&4.32&2.65&.27 \tabularnewline
TUR&1.48&.05&1.82&-.39 \tabularnewline
USA&4.68&1.62&2.95&.1 \tabularnewline
\bottomrule 

\end{tabularx}
\end{table}


==> Graph/mintax_hq_multi_decompo_wel_all_15.tex <==
\begin{table}[tbp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Multilateral HQ minimum taxation at 15\%: change in welfare}
\label{mintax_hq_multi_decompo_wel_all_15}
\begin{tabularx}{\linewidth}{lCCCC}

\toprule
{Country}&{$ \Delta $ Welfare (in \%)}&{Tax revenues contribution}&{Income contribution}&{Imbalance contribution} \tabularnewline
\midrule \addlinespace[\belowrulesep]
AUS&.05&.05&0&0 \tabularnewline
AUT&.07&.05&.01&.01 \tabularnewline
BEL&.44&.08&.32&.05 \tabularnewline
BGR&-.21&.03&-.21&-.03 \tabularnewline
CAN&0&.06&-.06&0 \tabularnewline
CHE&.04&-.02&.05&0 \tabularnewline
CHN&-.18&.02&-.19&-.01 \tabularnewline
CZE&.12&.03&.08&.01 \tabularnewline
DEU&.14&.07&.06&.01 \tabularnewline
DNK&.2&.09&.1&.01 \tabularnewline
ESP&.01&.07&-.07&0 \tabularnewline
FIN&.1&.08&.01&.01 \tabularnewline
FRA&.1&.08&.01&.01 \tabularnewline
GBR&.17&.09&.06&.02 \tabularnewline
GRC&-.45&.04&-.45&-.05 \tabularnewline
HKG&-.06&-.03&-.02&0 \tabularnewline
HRV&.03&.06&-.03&0 \tabularnewline
HUN&.26&.07&.16&.03 \tabularnewline
IND&-.18&.09&-.27&0 \tabularnewline
IRL&.03&-.07&.09&0 \tabularnewline
ISR&-.15&.05&-.19&-.01 \tabularnewline
ITA&-.05&.07&-.11&-.01 \tabularnewline
JPN&-.16&.05&-.21&-.01 \tabularnewline
KOR&-.04&.03&-.06&0 \tabularnewline
LTU&-.06&.03&-.08&-.01 \tabularnewline
LUX&-.28&-.34&.08&-.02 \tabularnewline
MEX&-.08&.05&-.12&0 \tabularnewline
MYS&.05&.04&0&0 \tabularnewline
NLD&-.08&-.11&.03&0 \tabularnewline
NOR&.16&.08&.09&-.01 \tabularnewline
NZL&-.18&.04&-.2&-.01 \tabularnewline
OFC&.01&-.08&.06&.02 \tabularnewline
POL&-.06&.03&-.07&-.01 \tabularnewline
PRT&-.12&.04&-.14&-.01 \tabularnewline
RUS&-.13&.04&-.18&.01 \tabularnewline
SGP&-.08&-.13&.05&0 \tabularnewline
SVK&.05&.02&.02&0 \tabularnewline
SWE&.22&.11&.1&.02 \tabularnewline
TUR&-.35&.04&-.36&-.03 \tabularnewline
USA&.11&.11&-.01&.01 \tabularnewline
\bottomrule 

\end{tabularx}
\end{table}


==> Quantax_Jun2024/3_PS_estimation.tex <==
\section{Estimating Profit Shifting}  \label{section_calib}

Taking our model to the data requires estimating several parameters. 
An essential step in our procedure is estimating profit-shifting flows, from which we can back out $\mathbb{P}_{ilh}$ through a set of structural relations in the model.\footnote{As typical in the literature, we assume that no profit is shifted out of tax havens ($\alpha_{lh}\to \infty$, when $h=l$). Therefore, we back out the profit-shifting shares for the residence $i$ and non-haven country $l$.}

Our identification strategy rests on two pillars. 
The first is a decomposition implied by our model, which we formalize in Proposition \ref{Pilhdecomp}.
We start by noting that equation (\ref{probafrechet}) describes the probability for a firm from $i$ to select the pair $lh$ to locate its production and book its post-tax profits. 
The firm can either report its profit in the source country ($h=l$) or shift profits from the source country to a tax haven ($h\neq l$).  
We denote by $\Pi_{ill}$ the total post-tax profits declared in $l$ by firms from $i$ producing in $l$ and by $PS_{ilh}$ post-tax profits shifted to $h$ by $i-$firms producing in $l$. 
Total profits - shifted or not - by firms from $i$ are denoted $\Pi_i\coloneqq \sum_l \Pi_{ill}+\sum_{lh} PS_{ilh}$, while $PS_{i}\coloneqq \sum_{lh}PS_{ilh}$ (resp. $PS_{ih}\coloneqq \sum_{l}PS_{ilh}$) represents total shifted profits by firms from $i$ (resp. from $i$ to $h$).
We use the separability of $\mathbb{P}_{ilh}$ across country pairs to derive accounting equations determining bilateral profit shifting. 
	\begin{prop}[Decomposition of $\mathbb P_{ilh}$]\label{Pilhdecomp}The following decomposition holds
		\begin{align}\label{eqpilhdecomp}
			\mathbb{P}_{ilh} = \mathcal P_i \times \zeta_{il} \times \chi_{lh} ~ \text{, for} ~ h \neq l,
	\end{align}
where $\mathcal P_i=\frac{PS_i}{\Pi_i}$ is the probability that firms headquartered in $i$ shift profits, $\zeta_{il}$ is the probability that a tax-avoiding firm headquartered in $i$ locates production in $l$ and $\chi_{lh}$ is the probability that a tax-avoiding firm producing in $l$ books its profits in $h$. 
	\end{prop}
The proof is provided in Appendix \ref{app_triangle_ps}.
This proposition states that to infer $\mathbb{P}_{ilh}$, it is enough to observe three simpler objects: $\mathcal{P}_i,\,\zeta_{il}$ and $\chi_{lh}$.

Our strategy's second pillar helps us identify these objects. 
First, we show that $\zeta_{il}$ can be recovered as a function of multinational production flows, of aggregated profit shifting in residence countries $i$ and in source countries $l$, and of $\tilde{\upsilon_1}$ and $\tilde{\upsilon}_2$. 
Intuitively, for profits to be shifted from $l$, production must occur in $l$. 
However, because production and paper profits have different elasticities, the patterns of shifted profits are a distorted representation of real activity (captured by MP shares): our model implies that this distortion is shaped by $\frac{\tilde{\upsilon}_2+1}{\tilde{\upsilon}_1+1}$ (see in Appendix \ref{app_algo}). 
Second, to pin down $\chi_{lh}$, we use the following ``triangle identities'': the profits from firms with residence in $i$ that are booked in a tax haven $h$ must match the profits that they shift from any source country $l$ where they operate to a given tax haven $h$.  
Since our data allows us to compute ${PS_{ih}}$, we can thus recover the share of profits shifted from $l$ to any $h$, i.e., $\chi_{lh}$. 



\begin{figure}
\begin{center}
	\begin{tikzpicture}[scale=2]
		\node[shape=circle,draw=black] (A) at (0,0) {i};
		\node[shape=circle,draw=black] (B) at (3,0) {l};
		\node[shape=circle,draw=black] (C) at (1.5, 2.5) {h};
	%	\node[shape=circle,draw=black] (D) at (0.75,1.25) {$h^\prime$};
		\path [->](A) edge node [below] {$\zeta_{il}$} (B);
		\path [->](B) edge node [right] {\color{red}$\chi_{lh}$} (C);
		\path [->](C) edge node [left] {$\frac{PS_{ih}}{PS_i}$} (A);
	%	\path [->](C) edge node [right] {} (D);
	%	\path [->](C) edge [bend right] node [left] {Correction for conduit FDI} (A);
	\end{tikzpicture}
	\\
	\small{$i$: headquarter \quad $l$: production \quad $h$: haven \\ 
 \begin{flushleft}
	    Note: $\frac{PS_{ih}} {PS_i}$ is estimated (section \ref{sub_ps_ih}), $\zeta_{il}$ is a function of $MP_{il},PS_i,PS_l,\frac{\tilde{\upsilon_1}+1}{\tilde{\upsilon_2+1}}$ (see the algorithm in Appendix \ref{app_algo}). $MP_{il}$ is observed (see Appendix \ref{app_data}), $PS_i,\textrm{ } and \textrm{ } PS_l$ are estimated (see section \ref{secPSestimate} and Appendix \ref{app_algo}), $\tilde{\upsilon_1}$ and $\tilde{\upsilon_2}$ are estimated (section \ref{main_elasticities}). \textcolor{red}{$\chi_{lh}$} is recovered using the triangle identities.
	\end{flushleft}}
\end{center}
\caption{Triangle of Profit Shifting}
\label{ps_triangle}
\end{figure}




The triangle identities are illustrated in Figure \ref{ps_triangle} and formalized in Proposition \ref{triangleprop}:
%
\begin{prop}[Triangle of Profit Shifting]\label{triangleprop}
The following holds
\begin{align}
	\label{calib_ps_3}\frac{PS_{ih}}{PS_i} = \sum_{l\ne h} \zeta_{il} \times \chi_{lh}.
\end{align}
\end{prop}
%
%The attractiveness of the source country
%l for tax-avoiding firms from $i$ is indirectly linked to the tax base and profit-shifting elasticities. 
%We show how $\zeta_{il}$ can be recovered as a function of multinational production flows and elasticities ${\upsilon_1}$ and ${\upsilon_2}$ in appendix \ref{app_algo}.
%The estimations of these elasticities and $PS_{ih}$, which determines $\eta_{ih}$ are detailed in the next section. 
The system shown in (\ref{calib_ps_3}) gives a set of $ (N-H) \times H$ equations, with $N-H$ the number of non-haven countries and $H$ the number of tax havens. 
Equipped with our estimates of ${PS_{ih}}/{PS_i}$ and $\zeta_{il}$, we can solve for the set of $\chi_{lh}$. Last, it should be noted that our estimates of  $PS_{ih}$ pin down $PS_{i}$ and thus $\mathcal P_i$.
%The key idea that we are operating in a closed system, namely one in $ih$ flows match with the combinations of $il$ and $lh$ flows, underlies the identification of the matrix of $\chi_{lh}$. 
Summarizing our methodology, as formalized in Propositions \ref{Pilhdecomp} and \ref{triangleprop}, $\mathbb{P}_{ilh}$ is readily obtained from $\mathcal P_i$, $\zeta_{il}$ and $\chi_{lh}$.  



\subsection{Data}\label{sub_data}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our baseline sample consists of 40 countries from 2010-2014, which accounts for 84\% of the world GDP in 2014. 
The sample includes seven major tax havens (Hong Kong, Ireland, Luxembourg, Netherlands, Singapore, Switzerland, and Offshore Financial Centers, an aggregate of smaller tax havens).
Our methodology to estimate profit shifting, elasticities, and frictions uses information on bilateral FDI income and multinational production as building blocks.
We also use other data sources in the analysis (tax rates, tax havens' policies, trade, profits, and other national accounts data). 
Details on the construction of the datasets and auxiliary sources of information are provided in the data Appendix \ref{app_data}. 

The bilateral FDI income dataset is the first source of information from which we compute profit shifting.\footnote{See also \citealp{UNCTAD_world_2015}, \citealp{Jansky2019}, or \citealp{vicard_profit_2022} for studies that use the FDI rate of returns in tax havens.}
We collect it from bilateral balance of payment data issued by Eurostat and the OECD. It corresponds to the income of foreign affiliates returned to their residence country through dividends, interests, or reinvested earnings. The profits shifted to tax haven affiliates are either returned to the high-tax country as dividends or counted as reinvested earnings (interest income follows a different pattern in profit shifting schemes, see \citealp{wright_exorbitant_2018}).
To construct our FDI income series, we add up the flows of reinvested earnings in tax havens and dividends from tax havens.
 	
The second important dataset is the multinational production (MP) dataset. 
This data allows us to construct $X_{ill}$, the sales resulting from the production in the country $l$ by firms headquartered in the country $i$. 
We use data on country-level production to compute production by domestic firms ($Q_{l}$).
We construct the MP data following \citet{ramondo2015multinational} using information on MNEs' bilateral sales from Eurostat, OECD, and the BEA.

In the following, we sketch our methodologies to calibrate profit shifting and the key elasticities. 
This procedure requires the calibration of $\sigma$ and $\iota_l$.
We use administrative French firm-level data from the FARE dataset and follow the methodology provided by \citet{deloecker2012markups} to estimate firm-level markups. 
The results give a median markup equal to 17\%, which corresponds to $\sigma=6.88$.\footnote{This is in line with estimates found in the literature, e.g., \citet{tintelnot2017global}. 
Similarly, \citet{deloecker2020rise} find a median markup of around 20 percent using Compustat data.}
With the estimation of $\sigma$, $\iota_l$ is then calibrated using the wedge between gross output and profits (corrected for profit shifting). Overall, $\iota_l$ absorbs any non-labor cost that impacts profits but not sales.
\begin{comment}
\subsection{Elasticity of substitution and profit rate \label{main_sigma}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The CES monopolistic competition set-up implies a markup equal to $\frac{\sigma}{\sigma-1}$. 
We use administrative French firm-level data from the FARE dataset and follow the methodology provided by \citet{deloecker2012markups} to estimate firm-level markups. 
The results give a median markup equal to 17\%, which corresponds to $\sigma=6.88$.\footnote{This is in line with estimates found in the literature, e.g., \citet{tintelnot2017global}. Similarly, \citet{deloecker2020rise} find a median markup of around 20 percent using Compustat data.}


With the estimation of $\sigma$, $\iota_l$ is then calibrated using the wedge between gross output and profits (corrected for profit-shifting). Overall, $\iota_l$ absorbs any non-labor cost that impacts profits but not sales.
%Expenditures on intermediate goods, fixed production costs are examples that all impact net profits but not sales.
\end{comment}
\subsection[Estimation of PS]{Estimation of $PS_{ih}$}\label{secPSestimate} \label{sub_ps_ih}
We now evaluate profit shifting from each headquarter country $i$ to each tax haven $h$, $ PS_{ih}$. We define profit shifting as the difference between the predicted FDI income and the counterfactual FDI income that would have been generated if there were no tax haven in our sample.
These counterfactual incomes are computed from an equation that regresses FDI income on factors related to gravitational forces, a tax haven indicator, and the effective average tax rate differential between pairs of countries:
\begin{eqnarray} \label{eq:fdi_income}
    FDI~Income_{jk}&=& exp(\beta_1 Haven_{k} +\beta_2 (ETR_j - ETR_{k}) \\
 \nonumber   &&+ \theta^{'} \bm{X_{jk}} + r_k + \mu_j) + u_{jk}. 
\end{eqnarray}
%
$FDI~Income_{jk}$ is the FDI income from an investment of country $j$ in country $k$. 
$Haven_{k}$ an indicator variable equal to 1 if country $k$ is a tax haven. $ETR_j - ETR_{k}$ is the effective average tax rate differential between country $j$ and $k$. $\bm{X_{jk}}$ represents a set of gravity variables and $\theta$ the vector of coefficients associated. $r_k$ are destination country's world region fixed effects, $\mu_j$ are investing country $j$ fixed effects, and $u_{jk}$ are the residuals.
We estimate equation (\ref{eq:fdi_income}) using the Poisson pseudo-maximum likelihood (PPML) estimator to take into account heteroskedasticity (\citealp{santos_silva_log_2006}) and to allow us to work with predictions in levels, avoiding the (log) OLS prediction's transformation issue (\citealp{duan_smearing_1983}).

Profit shifting from residence $i$ to a tax haven $h$, $PS_{ih}$, is defined as the difference between the predicted and counterfactual income that are predicted by muting the tax haven premium:
$  PS_{ih} = \reallywidehat{FDI~Income_{ih}} - \reallywidehat{FDI~Income_{ih}^0}$
with $\reallywidehat{FDI~Income_{ih}}$ the prediction of equation (\ref{eq:fdi_income}) on the sample of all pairs $ih$ composed of non-haven countries $i$ investing in tax havens $h$. $\reallywidehat{FDI~Income_{ih}^0}$ is defined on the same sample and corresponds to the predicted FDI income when the tax haven premium is set to 0 for all countries (i.e., $\beta_1=0$).

Table \ref{estimation_ps} presents the tax haven coefficients across different specifications 
(the complete estimation results are given in Appendix \ref{table1_full}).
We aggregate the amount of bilateral profit shifted that we report along with the share of aggregate profit shifting in the sample's total profit.
We use column (2) estimates to compute $PS_{ih}$. In particular, this specification includes Region $\times$ Tax Haven fixed effects to capture the geographical specialization of tax havens (\citealp{Laffitte_LTPS_2020}). 
The amount of profit shifting could be overstated because some tax havens, like The Netherlands, are used as intermediate locations from where profit might be transferred. 
We follow \citet{damgaard_phantom_2019} to correct the profit-shifting series from conduit-tax havens (see appendix \ref{app_conduit}). 

\begin{table}[ht]
		\caption{Estimation of $PS_{ih}$}
		\centering
		\label{estimation_ps} \footnotesize{
\begin{tabular}{lccccc} 
\toprule
	& \multicolumn{5}{c}{Dependent variable: $FDI~income_{jk}$} \\
\noalign{\smallskip}  \cline{2-6}\noalign{\smallskip} 
	& (1) & (2) & (3) & (4) & (5) \\ 
\noalign{\smallskip} \midrule \noalign{\smallskip} 
$ Haven_{k}$ & 1.565*** & 2.336*** & 2.767*** & 2.104*** & 1.677** \\
 & (0.227) & (0.238) & (0.337) & (0.747) & (0.669) \\
	\midrule
    Gravity Controls & Yes & Yes & Yes & Yes & Yes \\
	HQ FE & Yes & Yes & Yes & Yes & Yes \\
    HQ FE $\times$ Haven & No & No & No & Yes & Yes \\
	Destination Region FE & Yes & Yes & Yes & Yes & Yes \\
	Destination Region FE $\times$ Haven & No & Yes & Yes & Yes & Yes \\
	\midrule
	Observations & 1,444 & 1,444 & 1,444 & 1,444 & 1,212 \\
Pseudo R2 & 0.819 & 0.836 & 0.861 & 0.884 & 0.898 \\	
Destination countries & 52 & 52 & 52 & 52 & 52 \\ 
	\midrule
	\textbf{Implied Aggregate} 	\textbf{Profit Shifting} & \textbf{393551} & \textbf{397358} & \textbf{411327} & \textbf{408764} & \textbf{380954} \\
    Share sample's profits & 39\% & 40\% & 41\% & 41\% & 40\% \\ \bottomrule
\end{tabular}}
\caption*{\footnotesize{Note: In column (1), we assume that the tax havens' impact on FDI income is the same for all tax havens. 
In column (2), we include Region $\times $ Haven fixed effects assuming that tax havens are used differently according to their geographic location (\citealp{Laffitte_LTPS_2020}). 
Quadratic terms for distance and GDP are included in column (3).
In column (4), we allow the origin countries to have a different propensity to use tax havens (\citealp{desai_demand_2006}, \citealp{garcia-bernardo_uncovering_2017}) by including an interaction term between headquarter country fixed effects and the tax haven dummy variable.   
In column (5), we add a measure of the number of employees to account for labor inputs. Robust standard errors clustered at the destination country level in parentheses. *** p$<$0.01, ** p$<$0.05, * p$<$0.1. }}
	\end{table}

Once equipped with $PS_{ih}$, we can compute $PS^W:=\sum_{i,h}PS_{ih}$, the total amount of profit shifting. 
We estimate it to \$397bn, which corresponds to 39\% of all profits in the sample.  
This is in line with TWZ, that report a share of profit shifting that amounts to 36\% of global multinational profits. 
In Appendix \ref{rob_ps_u2_cbcr}, we provide alternative quantifications based on the OECD's Country-by-Country reporting (CbCR) data. 
With this alternative source, we also evaluate this share to be about 40\%. 

\subsection{Real activity and profit-shifting elasticities}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Armed with the estimated profit-shifting flows, we can use a first set of model relations to estimate the tax elasticities.
They will determine how changes in the global tax environment affect entry, production, and profit-shifting decisions. 
A novelty of our approach is to allow for, and calibrate, two tax elasticities: one for the tax base (governed by $\tilde{\upsilon}_1$) and one for profit shifting (governed by $\tilde{\upsilon}_2$). 
This allows corporate tax changes to induce different responses from real activities and profit shifting.
In addition, the model restrictions impose $\tilde{\upsilon}_2\geq \tilde{\upsilon}_1$, meaning that profit shifting is more elastic to taxes than real production (which is governed by both $\tilde{\upsilon}_1$ and $\tilde{\upsilon}_2$). 
This approach is motivated by the recent empirical corporate taxation literature, which emphasizes the non-linear responses of profits to corporate tax rates (e.g., \citealp{dowd_profit_2017}, \citealp{bratta_assessing_2021}, \citealp{fuest2021corporate}, \citealp{garcia2021profit}). 
These papers, however, do not distinguish between profits generated by production activities and shifted incomes. 
Instead, the elasticity is estimated using data that pool together tax havens (where a large share of profits are shifted) and high-tax countries.  
Conditional on real activity, their results suggest a larger impact of corporate tax rates on profits for countries with low tax rates than for countries with higher tax rates. 
This finding is consistent with our setting, where the elasticity of profit shifting to taxes is larger than that of real activity. 

To estimate the elasticities, we start by using Proposition \ref{gravityprop}, rewriting equations (\ref{gravitynoPSmodel}) and (\ref{gravityPSmodel}) in terms of observables and fixed effects.

\paragraph{Elasticity of the tax base.} 
The elasticity of the tax base in country $l$, $\tilde{\upsilon}_1$, is obtained by rearranging and estimating the logarithm of equation (\ref{gravitynoPSmodel}) as:
%\begin{align}
%	\frac{X_{ill}}{\sum_l X_{ill}}=\frac{\tilde{A}_{ill}(1-t_{ll})^{\frac{\upsilon_{1}}{\sigma-1}-1}}{\sum_{l}\tilde{A}_{ill}(1-t_{ll})^{\frac{\upsilon_{1}}{\sigma-1}-1}} \quad \forall (i,l) .\label{eq:FAS}
%\end{align}
%\begin{align}
%	\frac{X_{ill}}{\sum_l X_{ill}}=\frac{\tilde{A}_{ill}(1-t_{ll})^{{\tilde{\upsilon}_{1}}}}{\sum_{l}\tilde{A}_{ill}(1-t_{ll})^{{\tilde{\upsilon}_{1}}} }\quad \forall (i,l) .\label{eq:FAS}
%\end{align}
%$X_{ill}$ represents sales of firms from $i$, producing in $l$ and locating their profits in $l$.
%Taking the logarithm of (\ref{eq:FAS}), we obtain
\begin{align} \label{upsilon1_eqn}
\ln\left(\frac{X_{ill}}{\sum_lX_{ill}}\right)=\kappa_{0}\ \ln\left(1-{t}_{ll}\right)+\kappa_{1}\ \ln\tilde{A}_{ill} -\ln\left(\sum_{l}\tilde{A}_{ill}(1-t_{ll})^{\tilde{\upsilon}_{1}} \right), 
\end{align}
where $\kappa_0=\tilde{\upsilon}_1$ is our coefficient of interest.
$\tilde{A}_{ill}$ includes bilateral frictions between residence and source countries and the production market's wage level and size. 
The regression analysis includes total and per capita GDP (in logs) and gravity-related control variables such as distance, contiguity, and indicators for colonial relationships.
The headquarter country fixed effect is $FE_i= \ln\left(\sum_{l}\tilde{A}_{ill}(1-t_{ll})^{\tilde{\upsilon}_{1}} \right)$. 
We, therefore, use the variation across source countries to identify our coefficients.

\paragraph{Profit-shifting elasticity.}Taking the logarithm of (\ref{gravityPSmodel}), we obtain:
%
\begin{align} \label{gravitynoPSmodel_logbis}  
\ln\left(\frac{X_{ilh}}{\sum_{l,h,h\neq l}X_{ilh}}\right)=\delta_0 \ln(1-t_{lh}) + \delta_1 \ln \tilde{A}_{ilh} - \ln\left({\sum_{l,h,h\neq l}\tilde{A}_{ilh}^{\frac{1+\tilde{\upsilon}_{2}}{1+\tilde{\upsilon}_{1}}}(1-t_{lh})^{\tilde{\upsilon}_2}}\right),  
\end{align}
where $\delta_0= \tilde{\upsilon}_2 $ is our coefficient of interest. 
$t_{lh}$ is the tax rate applicable in tax haven $h$ to tax-avoiding firms producing in country $l$. 
This tax rate is not observed as tax havens generally offer legal dispositions that allow effective tax rates to differ from the observed statutory tax rate. 
We use the OECD's Country-by-Country reporting (CbCR) data to compute it. This data aggregates (mandatory) firm-level reports informing on the country-by-country breakdown of firms' accounting information, including taxes paid, turnover and profits. It is gathered by the OECD as part of the Action 13 of the BEPS project and targets large MNEs (revenues larger than 750 million euros).\footnote{This data has been used in other studies on tax avoidance by multinationals (\citealp{garcia2021multinational} at the macro level, \citealp{fuest2021corporate} or \citealp{bratta_assessing_2021} at the micro-level).}
The CbCR dataset is publicly available for a limited sample of 25 reporting countries.
We use this data to proxy the effective tax rate $t_{lh}$ ($h\neq l$) by the median effective tax rate observed in each tax haven, $t_{h}$.
In further exercises reported in section \ref{main_elasticities}, we show the robustness of the results using bilateral effective tax rates and alternative data sources.  

In Equation (\ref{gravitynoPSmodel_logbis}), $\tilde{A}_{ilh}$ comprises information about technology $A_{l}$; bilateral frictions between residence and source countries $\gamma_{il}$; between source countries and the tax havens, $\alpha_{lh}$; the source country's wage $w_l$ and market potential $\Xi_l$. The last term on the RHS of (\ref{gravitynoPSmodel_logbis}) is a headquarter fixed effect.
We add a set of headquarter $\times$ production country fixed effects, $FE_{il}$ and we parametrize the frictions $\alpha_{lh}$ between the source country $l$ and the tax haven $h$ with gravity covariates. 
We also add an index of the tax haven aggressiveness, taken from the TJN's Corporate Tax Haven Index (\citealp{CTHI}), to proxy for the tax avoidance ``technology'' of tax havens. 

As noted earlier, $\tilde{\upsilon}_2$ is needed to estimate profit shifting (see Section \ref{section_calib}) while it is also estimated using profit-shifting data. To determine its value, we follow an iterative procedure.\footnote{We guess a value of $\tilde{\upsilon}_2$, compute $\zeta_{il}$ and $PS_{ih}/PS_i$ and use (\ref{calib_ps_3}) to back out $\chi_{lh}$ and (\ref{eqpilhdecomp}) to compute $\mathbb{P}_{ilh}$. We then use the implied profit-shifting flows to update the guess on $\tilde{\upsilon}_2$ through (\ref{gravitynoPSmodel_logbis}) and iterate until convergence.}



\begin{comment}
To invoke Proposition $\ref{Pilhdecomp}$ and compute $\mathbb{P}_{ilh}$, we need $\zeta_{il}$ and $\chi_{lh}$. Proposition \ref{triangleprop} tells us that, given $PS_{ih}/PS_i$, it is enough to observe either $\zeta_{il}$ or $\chi_{lh}$ to infer the other. 
Intuitively, $\zeta_{il}$ relates to the multinational activity by tax-avoiding firms. 
Our model provides a tight relationship between $\zeta_{il}$ and the multinational production share together with the elasticities $\tilde{\upsilon}_1,$ and $\tilde{\upsilon}_2 $. 
Given our estimated elasticities, data on multinational production, and data on aggregated profit-shifting in residence countries $i$ and in source countries $l$, we back out $\zeta_{il}$. 
Next, we use our matrices of $PS_{ih}/PS_i$ and $\zeta_{il}$ to compute the set of $\chi_{lh}$ through equation (\ref{calib_ps_3}). 
We detail our $\zeta_{il}$ calculation in the Appendix \ref{app_algo}. 
Finally, having obtained $\mathcal{P}_i,\,\zeta_{il}$ and $\chi_{lh}$, we can use Proposition \ref{Pilhdecomp} to compute our object of interest $\mathbb{P}_{ilh}$ (see, Appendix \ref{app_estimation_PS} for technical details).
\end{comment}

We summarize the methodology covered in this section before diving into the analysis of our empirical results. 
Given profit shifting and multinational production flows, we can i) estimate the elasticities $\tilde{\upsilon_1}$ and $\tilde{\upsilon}_2$, ii) compute the probability that a firm from $i$ shifts profits $\mathcal{P}_i$,
iii) use data on multinational production and the elasticity to compute the probability that a tax-avoiding firm from $i$ locates production in $l$, $\zeta_{il}$, iv) use our ``triangle identities'' to back out the probability that a firm, producing in $l$, shifts profits to $h$, $\chi_{lh}$; and v) use our decomposition in $(\ref{eqpilhdecomp})$ to compute $\mathbb{P}_{ilh}$.


==> Quantax_Jun2024/4_PS_frictions.tex <==
\section{Profit-Shifting Flows, Elasticities and Frictions} \label{section_elasticities}
In this section, we discuss our empirical results. 
We start by describing the estimated profit-shifting flows and their implied elasticities. 
Finally, we illustrate our estimates of the profit-shifting frictions.




\subsection{Profit-Shifting Flows \label{main_ps}}

The diagram in Figure \ref{fig:sankey_lh} displays the estimated profit that has been shifted to tax havens (in the center) according to the residence country (on the left) and the source country (on the right).
For visualization, we display the top 10 countries and aggregate the bilateral shares for others. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.65\linewidth]{Graph/sankey_ilh.png}
	\caption{Profit shifting shares from residence-country $i$ to $h$ ($PS_{ih}/PS_i$)\\ and from source-country $l$ to $h$ ($\chi_{lh}$).}
	%\caption*{\footnotesize Note: This figure displays the estimated profit that has been shifted to tax havens (in the center) according to the residence country (on the left) and the source country (on the right).}
	\label{fig:sankey_lh}
\end{figure}

The figure shows the predominance of residence countries such as the U.S. and, to a lesser extent, Germany, the UK, and France in shifting profits to tax havens. 
It also shows the importance of European tax havens and, in particular, the Netherlands as a major destination for profit shifting.
Furthermore, Figure \ref{fig:sankey_lh} suggests larger shares of profit shifted from the U.S. as a residence country than as a source.  
This is also the case for France, Germany, and the United Kingdom but not Japan and China.
The pattern displayed in Figure \ref{fig:sankey_lh} confirms that gravitational frictions shape profit shifting.
European tax havens prominently host profits from non-haven countries in the E.U. and the U.S., while China and Japan shift most of their profits to Hong Kong and Singapore. 

\paragraph{Comparisons.} 

Several papers provide estimates of profit shifting at the production country or tax haven level (\citealp{zucman_taxing_2014}, \citealp{clausing_effect_2016, clausing_2020}, \citealp{Jansky2019}, \citealp{garcia2021profit} and \citealp{torslov_missing_2022}).
\citet{torslov_missing_2022} is the first paper to propose a methodology to compute bilateral profit shifting across pairs of source and tax haven countries.
They use the global amounts of shifted profits and an allocation key based on trade in high-risk services to determine profit-shifting between source countries and tax havens.\footnote{In Appendix's section \ref{app_ps_stateoftheart}, we briefly discuss the approach followed so far by the literature and, especially TWZ. We argue that profit shifting in goods, tax-havens deflated imports and non-``high-risk'' services are three additional sources that come on top of the excess of ``high-risk'' services exports and intra-firm interest payments considered in TWZ. We also discuss the robustness of our calibration using inputs from TWZ in Appendix's section \ref{PS_robustness}.} 
While the relative rank of source countries using different methodologies proves to be similar, we find the relative position of country pairs regarding profit shifting to be less correlated.  


%We highlight two reasons for which we prefer the approach developed in section \ref{section_calib} for our baseline calibration: sample compatibility and (the lack of) assumptions about the sources of profit-shifting. 


%TWZ's bilateral allocation of profit-shifting mainly relies on bilateral trade in services. In Appendix \ref{comparison}, we provide some evidence that the contribution of non high-risk services may have been underestimated. We argue that profit-shifting in goods, tax-havens deflated imports; and high-risk services matter as well for the allocation of bilateral shifted profits. 


We benchmark our shifted profit flows with these previous estimates. 
Table \ref{correlations} reports Spearman's rank correlations of our vector of estimated profit shifting with different estimates from the literature. 
In Panel A, we aggregate our bilateral measure of profit shifting for each production country and display the correlations of this vector with unilateral profit-shifting measures constructed by TWZ, the Tax Justice Network (\citealp{tjn_2020}), and the European Commission using the CORTAX model (\citealp{cortax2016}). 
We find large positive rank correlations at the unilateral level, suggesting a stable relative position of each source country in profit shifting irrespective of the methodology used. 

\begin{table}[ht] 
	\centering
	\small
	\caption{Spearman's rank correlation}
	\label{correlations}
	\begin{tabular}{lcc} \toprule
		Source& Correlation &  Obs. \\ 
		\midrule
		A. Unilateral profit shifting: \\
		\noalign{\smallskip}  \cline{1-1}    \noalign{\smallskip}
		\citet{torslov_missing_2022}  & 0.90& 33 \\
		\citet{tjn_2020} & 0.92 & 33\\
		\citet{cortax2016}  & 0.95 & 21\\ 
		\midrule
		B. Bilateral profit shifting: \\
		\noalign{\smallskip}  \cline{1-1}    \noalign{\smallskip}
		\citet{torslov_missing_2022}  & 0.61	 & 111 \\
		\noalign{\smallskip}  \hline    \noalign{\smallskip}

	\end{tabular}
\end{table}

In Panel B, we compare our estimations with the bilateral estimates of \citet{torslov_missing_2022}.
We restrict our comparison to bilateral estimates for European tax havens as TWZ reports an aggregate for non-European tax havens.
We find a strong rank correlation between our bilateral measure and the one of TWZ, slightly above 60\%.
TWZ's bilateral allocation of profit shifting mainly relies on exports of services by tax havens.
In contrast, we are agnostic about the channels of profit shifting (see section \ref{app_ps_stateoftheart} of our Appendix for a discussion). In our Appendix's section \ref{comparison}, we provide additional material that compares our profit-shifting estimates with other sources found in the literature. 

Finally, we propose different robustness exercises in our Appendix's section \ref{PS_robustness}. We assess the correlation between our profit-shifting allocation and an allocation based on excess trade in services with tax havens only. We find a positive and significant correlation between excessive high-risk services and our theoretically consistent measure of bilateral profit shifting. The Spearman rank correlation coefficient of 0.6 indicates a relatively high correlation between both series but the $ PS_{lh}$ estimated in this paper is generally larger than the excess of services trade.
This result suggests that services trade is an important driver of profit shifting between source countries and tax havens but shall not be considered its unique determinant.\footnote{
In Appendix Figure \ref{fig:ps_il_robustness_upsilon}, we explore the role of the parameters $\tilde{\upsilon}_1$ and $\tilde{\upsilon}_2$ on the allocation of profit shifting and find that the estimated profit shifting is robust to different calibrations of these elasticities.}

\subsection{Tax Base and Profit-Shifting Elasticities \label{main_elasticities}}
Table \ref{reg_u1u2} reports the estimated coefficients and the corresponding parameter elasticities $\tilde{\upsilon}_1$ and $\tilde{\upsilon}_2$.
%for our estimated value of $\sigma=6.88$ and for a lower estimate of $\sigma=4$ for comparability with other studies.
In columns (1) and (2), we use the statutory tax rates as the corporate tax variable, while we use the median effective tax rate in columns (3) and (4).
We report the result using OLS in columns (1) and (3), and PPML in columns (2) and (4). 
%
\begin{table}[ht]
	\centering
 	\caption{Estimation of elasticities $\tilde{\upsilon}_1$ and $\tilde{\upsilon}_2$\label{reg_u1u2}}
\begin{tabular}{l@{\extracolsep{0.05in}}cccc} \toprule
& \multicolumn{2}{c}{Estimation $\tilde{\upsilon}_1$} & \multicolumn{2}{c}{ Estimation $\tilde{\upsilon}_2$} \\ 
\noalign{\smallskip} \cline{2-3} \cline{4-5}\noalign{\smallskip} 
Dep. Var. &  $ln\left(\frac{X_{ill}}{\sum_i X_{ill}}\right)$ &$\frac{X_{ill}}{\sum_i X_{ill}}$ &  $ln\left(\frac{X_{ilh}}{\sum_i X_{ilh}}\right)$   & $\frac{X_{ilh}}{\sum_i X_{ilh}}$    \\ 
\noalign{\smallskip} \cline{2-3} \cline{4-5}\noalign{\smallskip} 
& (1) & (2) & (3) & (4) \\
\noalign{\smallskip} 
\noalign{\smallskip} \cline{1-3} \cline{4-5}\noalign{\smallskip} 
\noalign{\smallskip} 
	$ ln(\tilde{t}_{ll}) $  &  2.639*** & 3.047*&& \\
	& (0.688) & (1.674)&& \\
	$ ln(\tilde{t}_{lh}) $ (Med.)&& & 7.869*** & 8.625*** \\
	&&& (0.191) & (1.295) \\ 
 \midrule
	Observations & 1,256 & 1,600 & 6,561 & 7,091  \\
	Estimator & OLS & PPML  & OLS & PPML\\ 
 \midrule
	Gravity controls & Yes  & Yes & Yes & Yes \\ 
	$i$ country FE & Yes & Yes & No & No  \\
	\textit{i-l} pair FE & -- &-- & Yes & Yes  \\
	Technology controls & Yes & Yes & -- & -- \\ 
 %\midrule
	%$ \sigma $ = 4     & 10.90 & 12.10 & 26.60 & 28.90 \\
	%$ \sigma $ = 6.88  & 21.40 & 23.80 & 52.10 & 56.60\\
 \bottomrule
\end{tabular}
\caption*{\footnotesize Note: Robust standard errors clustered at the $i \times l$ level in parentheses. Gravity controls include bilateral distance (in logarithm), a contiguity dummy, colonial linkages dummies, common legal origin dummies, and common language dummies. Technology controls include GDP and GDP per capita (both in logarithm). Our main estimate of $\tilde{\upsilon}_2$ (column (3)) is estimated following an iterative procedure where we first guess a value of $\tilde{\upsilon}_2$, compute $\zeta_{il}$ and $PS_{ih}/PS_i$ and use (\ref{calib_ps_3}) to back out $\chi_{lh}$ and (\ref{eqpilhdecomp}) to compute $\mathbb{P}_{ilh}$. We then use the implied profit-shifting flows to update the guess on $\tilde{\upsilon}_2$ through (\ref{gravitynoPSmodel_logbis}) and iterate until convergence. *** p$<$0.01, ** p$<$0.05, * p$<$0.1.}
\end{table}
%

We find a profit-shifting elasticity, $\tilde{\upsilon}_2=7.9$, three times the tax base elasticity, $\tilde{\upsilon}_1=2.6$. Our estimate suggests that multinational production - which is governed by both elasticities - is relatively mobile across countries.\footnote{The elasticity of production to MP-frictions  $\upsilon_1$ would have been $10.9$ assuming $\sigma=4$. 
It is somewhat larger than the elasticity found in the literature.
For comparison, \citet{head2019brands} and \citet{wang2020multinational} estimate an elasticity of 7.7.  
This implies that the impact of multinational firms' production and profit-shifting frictions will be downplayed in our quantitative exercises compared to these estimates. For comparability purposes, in table \ref{semi-elasticities} of Appendix \ref{semi-elasticities_section}, we also compute the semi-elasticity of the tax base to taxes and of profit shifting to taxes using the same specification as in Table \ref{reg_u1u2}. We find a semi-elasticity of the tax base of 3.6 and of profit shifting of 8.3. In their meta-study, \citet{international_beer_2020} find that the average semi-elasticity
of profits to taxes estimated in studies that use aggregate data is between 2.5 (Table 2, column 3) and 2.9 (Table 2, column 2). Our semi-elasticity of the tax base to taxes, despite being slightly higher than this average, lies in the same range. In their estimation of a non-linear elasticity of profit to taxes using micro-level country-by-country reporting data, \citet{fuest2021corporate} find a semi-elasticity of profits to taxes between -10 and -13 when the effective tax rate is close to zero, a situation which typically corresponds to tax haven affiliates. This result confirms large elasticities for profits (essentially paper profits) located in tax havens. We assess the sensitivity of our counterfactual experiments to alternative calibrations of $\tilde{\upsilon}_1$ and $\tilde{\upsilon}_2$ in section \ref{sup_mat_sensitivity} of the Appendix.}

\paragraph{Profit-shifting elasticity: Robustness.}
Overall, there is no direct comparison between our estimate of the profit-shifting elasticities and the literature. 
\citet{international_beer_2020} show in their meta-analysis that, all else equal, a 1-point decrease in the tax rate corresponds to an increase in reported profits by 1\%. 
In addition, a few studies have estimated the \textit{elasticity} of reported profits to corporate taxes using country-level data. 
\citet{gruber_elastic_2007} find a moderate elasticity of the corporate tax base with respect to current effective tax rates (equivalent to 0.2).
Using administrative data on U.S. tax filings, a recent study by \citet{coles_how_2022} decomposes the corporate tax elasticity of taxable income into a tax base and a paper profit elasticity.  
In line with our findings, their results suggest larger profit-shifting reactions to corporate tax than tax-base responses. 

So far, our estimation relies on the profit-shifting flows we estimated following the methodology of section \ref{section_calib}. 
To assess the sensitivity of our implied elasticities, we use alternative data sources of income and profit shifting, effective tax rates, and different methodologies. 
First, we reproduce the results shown in column (4) of Table \ref{reg_u1u2} by using direct information on profit shifting from source to haven countries from \citet{wier_global_2022}. 
Second, we reproduce the results of Table \ref{reg_u1u2} by using the information on bilateral effective tax rates for the 25 countries reporting in the OECD CbCR dataset.
Third, we construct a new sample of bilateral reported pre-tax income and bilateral effective tax rates using micro-level data from the Refinitiv Thomson Reuters \emph{Eikon} database – hereafter, the Eikon dataset. 
The dataset allows us to use high-dimensional fixed effects and control for unobserved bilateral frictions determining excess profits. 
It has, however, the drawback of covering only a few countries, particularly tax havens.
Details on sample construction are provided in Appendix \ref{rob_ps_u2_cbcr}. 

Using data from \citet{torslov_missing_2022} allows a direct estimation of $\tilde{\upsilon}_2$ while the other two sources require us to estimate shifted profits. 
Therefore, we proceed in two steps using the CbCR and Eikon datasets.
In the first step, we estimate the amounts of profit shifted to tax havens.
The empirical specification includes bilateral ETRs, gravity controls, and a set of origin $\times$ year and destination $\times$ year fixed effects, removing country-specific and time-varying unobserved heterogeneity.
Under this fixed effect specification, we cannot identify excess profits based on the tax haven dummy.
We follow the methodology proposed by \citet{garcia2021profit}, who compute profit shifting to tax havens based on the hypothetical case that tax havens would have had an effective tax rate (ETR) of 25\%.
Profit shifting is computed as the difference between the predicted profits and those predicted with the counterfactual tax rates of 25\%. 
In the second step, we regress profit shifting on the $\log(1-t_l^{ETR})$, gravity controls, and a set of origin $\times$ year and destination $\times$ year fixed effects following the specification of equation (\ref{gravityPSmodel}). 
When time variation allows, we include pair-fixed effects in both steps.

Table \ref{u2_rob_maintext} reports a summary of our results. 
The complete estimation table is reported in Appendix \ref{rob_ps_u2_cbcr}. 

\begin{table}[ht]		
\begin{center}	
	\caption{Alternative identification of $\tilde{\upsilon}_2$}
	\label{u2_rob_maintext}
 \begin{tabular} {lcccc}			
	\noalign{\smallskip}  \hline \noalign{\smallskip}			
	& (1) & (2) & (3) & (4)	 \\ \noalign{\smallskip}												

	Data Source	&	WZ	&	CBCR	&	Eikon	&	Eikon	\\
 	\noalign{\smallskip}  \hline \noalign{\smallskip}												

	Implied $\tilde{\upsilon}_2$ &	10.5	&	8.2	&	8.4	&	5.4	\\
	\noalign{\smallskip}  \hline \noalign{\smallskip}												
Controls and FE in first and second steps		&		&		&		\\
\cline{1-1}
Gravity Controls	&	Yes	&	Yes	&	Yes	&	No	\\
Origin $\times$ Year FE	&		&	Yes	&	Yes	&	Yes	\\
Destination $\times$ Year FE	&		&	Yes	&	Yes	&	Yes	\\
Pair FE	&		&	No	&	No	&	Yes	\\
\noalign{\smallskip} \hline \noalign{\smallskip}
\end{tabular}											
\parbox{14.7cm}{\footnotesize Note: This table displays alternative estimations of profit shifting and corresponding estimation of $\tilde{\upsilon}_2$. In column (1), we directly use profit-shifting data from \citet{wier_global_2022} (WZ). In column (2), we estimate profit shifting using data from Country-by-country reports (CbCR), and in columns (3) and (4), we use the Eikon dataset. Details on the estimation procedure, additional results, and full tables are provided in Appendix \ref{rob_ps_u2_cbcr}. }\\
\end{center}											
\end{table}

In column (1), we use the TWZ estimate of profit shifting to compute $\tilde{\upsilon}_2$ following the specification of table \ref{reg_u1u2}.
In column (2), we use the bilateral ETR computed from the CbCR dataset and assume a constant profit elasticity to the effective tax rate.\footnote{In Appendix \ref{rob_ps_u2_cbcr}, we follow \citet{hines_fiscal_1994}, \citet{dowd_profit_2017} \citet{garcia2021profit} and allow for non-linearities. The results are qualitatively the same.}
We report the results using the Eikon dataset in columns (3) and (4).
Compared to column (3), column (4) reports results using pair fixed effects in addition to origin $\times$ year and destination $\times$ year fixed effects. 
Using alternative samples and calibration, we find that $\tilde{\upsilon}_2$ varies between 5.4 and 10.5 compared to $\tilde{\upsilon}_2=7.9$ in the baseline estimation.

In additional results shown in Appendix \ref{rob_ps_u2_cbcr}, we find that the ratio of profit shifting to total incomes in most samples matches our previous estimates at around 40\% of total incomes. 
We find lower estimates using the aggregated micro-level dataset because it is composed of fewer tax havens. 
Moreover, only a few firms report profits in tax-haven countries. 

\paragraph{Extension: varying profit-shifting elasticity.} \label{nonlinear_elasticity_main}

Our calibration of $\tilde{\upsilon}_2$ rests on the assumption that the share of profits shifted to tax havens is a constant elasticity function of the corporate tax rate. 
While this assumption is reasonable for small changes in corporate tax rates, policies like a minimum taxation reform could generate large variations in effective tax rates and tax rate differentials. 
We refine our parametrization of the profit-shifting elasticity and allow for an additional variable profit-shifting elasticity.   
We augment our profit-shifting friction $\alpha_{lh}$ with $\left(t_l-t_{lh}\right)^k$ where $k$ is a shape parameter.
The partial elasticity of profit shifting then becomes $\tilde{\upsilon}_2+\frac{k (1+\tilde{\upsilon}_2)}{1+\tilde{\upsilon}_1} \frac{(1-t_{lh})}{(t_l-t_{lh})}$. The shape parameter $k$ is recovered from the data (see results in Table \ref{reg_u2_k}). %\footnote{Alternative functional forms such as the simple differential $t_l-t_h$ do not yield an equally good fit but lead to similar results.}
The estimated $k$ is such that the elasticity is below $\tilde{\upsilon}_2$ for tax rate differentials above 20 percentage points.
This property will have implications for the implementation of the minimum tax rate.\footnote{A higher rate would reduce profit shifting more than proportionally. 
We observe large elasticities for tax differentials that are smaller than 10\%.
This result suggests larger responses of profit shifting when the tax differential is small.}
We implement this varying profit-shifting elasticity to simulate minimum taxation policy scenarios.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Profit-shifting frictions \label{main_frictions}} 

Bilateral profit-shifting frictions are an important novel ingredient of our framework. They govern how multinational firms decide whether and where to shift profits and produce. In this subsection, we back out these frictions, consistently with the observed flows of shifted profits by firms in residence $i$ to tax haven $h$ from source country $l$. 
We first detail the procedure and then explore the magnitude and determinants of these frictions.

\paragraph{Identifying Profit-shifting frictions.}
We start by noting that, at the calibrated equilibrium, we know profit-shifting probabilities
$\mathbb{P}_{ilh}$, taxes $t_{ll}$
and $t_{lh}$, and our estimated elasticities $\tilde{\upsilon_{1}},\tilde{\upsilon_{2}}$ (see Appendix \ref{appendix_ps_frictions} for details).
We formalize the identification result for profit-shifting frictions in the next Proposition. 

\begin{prop} [Identifying Profit-Shifting Frictions] {\ \\} At the calibrated equilibrium the following holds 
\begin{align} \label{frictioneq} 
\bar\theta\tilde\theta_i\alpha_{lh} \left(\frac{1-t_{ll}}{1-t_{ilh}}\right)^{\frac{1}{\sigma-1}}=\left(\frac{\mathbb{P}_{ilh}}{\mathbb{P}_{ill}}\right)^{-\frac{1}{\upsilon_1}}\left(\frac{\mathbb{P}_{ilh}}{\mathcal{P}_i}\right)^{\frac{1}{\upsilon_1}-\frac{1}{\upsilon_2}},\end{align} 
where $\bar{\theta}$ is a normalizing constant such that $\theta_i=\bar{\theta}\tilde{\theta}_i$. We specify $\bar\theta$ in Appendix \ref{appendix_ps_frictions}. \end{prop}

On the right-hand side of equation (\ref{frictioneq}), we have observable profit-shifting flows. On the left-hand side we have the tax differential gain of firms from $i$ producing in $l$ choosing to shift to haven $h$ rather than booking profits domestically in $l$. Given our previous definitions, we know that  $\left(\frac{\mathbb{P}_{ilh}}{\mathcal{P}_i}\right)^{\frac{1}{\upsilon_1}-\frac{1}{\upsilon_2}}$<1. Typically, in the data, $\left(\frac{\mathbb{P}_{ilh}}{\mathbb{P}_{ill}}\right)^{-\frac{1}{\upsilon_1}}>1$ as less profits are shifted than booked domestically. We also know that tax gains are typically such that $\left(\frac{1-t_{ll}}{1-t_{ilh}}\right)^{\frac{1}{\sigma-1}}$<1 as $t_{ll}$ is typically larger than $t_{ilh}$. Our frictions $\bar\theta\tilde\theta_i \alpha_{lh}$ are what we need to explain the observed PS flows, given the observed tax differential and elasticities. Whenever $\mathbb{P}_{ilh}$ is very large relative to $\mathbb{P}_{ill}$, the model will call for small profit-shifting frictions to rationalize the data. Importantly, frictions can be both above and below 1, depending on whether the tax differential gain is sufficient to explain observed profit-shifting flows. 

We note that $\tilde\theta_i=\theta_i/{\bar \theta}$ and $\alpha_{lh}$ can be mapped into a marginal cost equivalent $Cost_{ilh}\coloneqq \tilde\theta_i\alpha_{lh}$. This is the marginal cost increment associated with profit
shifting from any $l$ to any $h$ by firms from $i$ \emph{if
all profit-shifting frictions were such that $\alpha_{l'h'}=\alpha_{lh}$}.
In contrast with trade or multinational
production frictions, the interaction of the tax base
and profit-shifting elasticities implies that bilateral profit-shifting
flows do not verify the irrelevance of independent alternatives. The
cost of shifting profits from $l$ to $h$ depends on the profit-shifting frictions between other $l'-h'$ pairs.

\paragraph{Average profit-shifting costs.}
We start by describing the distribution of average $Cost_{ilh}$ between $l$ and $h$ in Figure \ref{fig:costps}. 
We plot the distribution of the profit-shifting cost averaged over (non-haven) $i$ countries: $Cost_{lh}=\frac{1}{33}\sum_i Cost_{ilh}$.

	\begin{figure}[!ht]
	\centering	
 \includegraphics[width=0.7\linewidth]{Graph/distrib_cost_lh_mean} 
		\caption{Average cost of profit shifting ($Cost_{lh}$)} \label{fig:costps}
	\end{figure}

Conditional on observing profit shifting, the median value of profit-shifting costs calculated in our sample is 1.23. It can be up to 1.5 for some pairs. 
A profit-shifting cost of 1.23 means that shifting from a residence country $i$ to a tax haven $h$ through a production affiliate $l$ generates an increase in the cost of production of 23\%, all other things being equal. 
The friction can be compared to the variable friction $\gamma_{il}$, which represents the costs of separating the location of production from headquarters. 
We find a median value of $\gamma_{il}$ of 1.40, similar to the multinational production costs of 1.31 provided by \citet{head2019brands} for the car industry. 

Given the magnitude of our estimated frictions, one should wonder why we observe any profit shifting since, for most triplets, the cost of shifting is higher than the tax advantage. For a given pair, frictions larger than the tax advantage reveal that the median firm does not shift profits. The firms who do book profits in tax havens are the selected ones for which the payoff of booking profits in tax havens is both the tax advantage $(1-t_{ilh})/(1-t_{ll})$ and their relative technology draw $\varphi_{lh}/\varphi_{ll}$. Whenever the technology advantage is large, firms might find it profitable to shift even if the frictions are large. In this sense, our model replicates salient empirical findings on firms' selection into profit shifting (\citealp{davies_knocking_2018}, \citealp{bilicka_comparing_2019}, \citealp{wier_2020jpube}, \citealp{wier_dominant_2023}).

 
\paragraph{Components of profit-shifting costs: $\tilde{\theta}_{i}$ and $\alpha_{lh}$.}
The profit-shifting cost has two components: the tax aggressiveness of the residence country $\tilde{\theta}_{i}$ and the bilateral friction $\alpha_{lh}$.
Our model suggests that the costs are separable via a fixed effect for $i$ and one for $lh$ pairs: $ln(Cost_{ilh})=ln(\tilde{\theta_i})+ln(\alpha_{lh})$. 
The residence country fixed effects correspond to the log of $\tilde\theta_{i}$. 
The source and tax haven dyadic fixed effects capture the bilateral profit-shifting frictions $\alpha_{lh}$.
About 27\% of the variation in profit-shifting costs is explained by the (log) bilateral frictions, $\alpha_{lh}$.
\footnote{Note that the different abilities of each residence country to reduce the costs of shifting profits should be interpreted as deviations from the tax aggressiveness of one reference country that we choose to be the U.S.}

In Figure \ref{fig:theta_i}, we show the cross-country distribution of $\ln\theta_{i}$. 
Compared to U.S. MNCs, Turkish firms experience a profit-shifting cost penalty of 35\%.
Belgian MNCs benefit from a 13\% reduction in profit-shifting costs compared to U.S. MNCs.  
The differences in tax aggressiveness across residence countries in Figure \ref{fig:theta_i} show the key role of headquarters in firms' profit-shifting practices. 

\begin{figure}[!ht]
\centering
		\includegraphics[width=0.7\linewidth]{Graph/ln_theta_i} 
		\caption{Distribution of $ln(\theta_i)$} \label{fig:theta_i}
	\end{figure}

Finally, we regress the log of $\alpha_{lh}$ on gravitational variables, tax rates, and the TJN’s Corporate Tax Haven index (CTHI). This last variable corresponds to an index computed by the TJN that aggregates 20 \textit{de jure} and \textit{de facto} indicators of the aggressiveness of tax havens' policies. We see it as a proxy for tax avoidance technology provided by tax havens (see Appendix \ref{app_tjn} for details).
We show in the Appendix Table \ref{table_costPS} that the distance between the source and tax haven countries, and other gravitational forces affect $\alpha_{lh}$. In other words, profit shifting frictions shape the geographic incidence of international tax reforms.
Moreover, profit-shifting frictions are negatively correlated with the TJN’s Corporate Tax Haven Index and with the corporate tax rate difference between the source and the havens.
We also find a negative correlation between the difference in tax rates of the source and haven countries and the profit-shifting friction, controlling for source and haven fixed effects.
This points to the importance of introducing a varying profit-shifting elasticity as done in Section \ref{main_elasticities}.


\begin{comment}
\paragraph{Determinants of profit-shifting costs.}
We start by describing the distribution of average $Cost_{ilh}$ between $l$ and $h$ in Figure \ref{fig:costps}.
Conditional on observing profit-shifting, the median value of profit-shifting costs calculated in our sample is 1.23. 
A profit-shifting cost of 1.23 means that shifting from a residence country $i$ to a tax haven $h$ through a production affiliate $l$ generates an increase in the cost of production of 23\%, all other things being equal. 


\begin{figure}[htbp]
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Graph/distrib_cost_lh_mean} 
		\caption{Average cost of profit-shifting ($Cost_{lh}$)} \label{fig:costps}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Graph/ln_theta_i} 
		\caption{Distribution of $ln(\theta_i)$} \label{fig:theta_i}
	\end{subfigure}
 \caption*{\footnotesize Note: Panel (a) plots the distribution of the profit-shifting cost averaged over (non-haven) $i$ countries: $Cost_{lh}=\frac{1}{33}\sum_i Cost_{ilh}$. Panel (b) plots the residence country fixed effects that theoretically corresponds to $ln(\theta_i)$.}
\end{figure}


The friction can be compared to the variable friction $\gamma_{il}$, which represents the costs of separating the location of production from headquarters. 
We find a median value of $\gamma_{il}$ of 1.40, similar to the multinational production costs of 1.31 provided by \citet{head2019brands} for the car industry. 

The profit-shifting cost has two components: the tax aggressiveness of the residence country $\tilde{\theta}_{i}$ and the bilateral friction $\alpha_{lh}$.
Our model suggests that the costs are separable via a fixed effect for $i$ and one for $lh$ pairs: $ln(Cost_{ilh})=ln(\tilde{\theta_i})+ln(\alpha_{lh})$ with $ln(Cost_{ilh})$, the logarithm of the profit-shifting costs. 
The residence country fixed effects correspond to the log of $\tilde\theta_{i}$. 
The source and tax haven dyadic fixed effects capture the bilateral profit-shifting frictions $\alpha_{lh}$.
About 27\% of the variation in profit-shifting costs is explained by the (log) bilateral frictions, $\alpha_{lh}$.
\footnote{Note that the different abilities of each residence country to reduce the costs of shifting profits should be interpreted as deviations from the tax aggressiveness of one reference country that we choose to be the U.S.}

In Figure \ref{fig:theta_i}, we show the cross-country distribution of $\ln\theta_{i}$. 
Compared to U.S. MNCs, Turkish firms experience a profit-shifting cost penalty of 35\%.
Belgian MNCs benefit from a 13\% reduction of profit-shifting costs.  
The differences in tax aggressiveness across residence countries in Figure \ref{fig:theta_i} show the key role of headquarters in firms' profit-shifting practices. 

We conclude with the examination of bilateral profit-shifting frictions. 
We regress the log of $\alpha_{lh}$ on gravitational variables, tax rates, and the TJN’s Corporate Tax Haven index (CTHI). 
We show in the Appendix Table \ref{table_costPS}, that distance between the source and tax haven countries, and other gravitational forces determine $\alpha_{lh}$. 
Moreover, profit-shifting frictions are negatively correlated with the TJN’s Corporate Tax Haven indexes and with the corporate tax rate difference between the source and the havens.
We also find a negative correlation between the tax rate difference of the source and haven countries and the profit-shifting friction.
This finding points to the importance of introducing a varying  profit-shifting elasticity.

\end{comment}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
